Powering In-Database Dynamic Model Slicing for Structured Data Analytics

Relational database management systems (RDBMS) are widely used for the storage of structured data. To derive insights beyond statistical aggregation, we typically have to extract specific subdatasets from the database using conventional database operations, and then apply deep neural networks (DNN) training and inference on these subdatasets in a separate analytics system. The process can be prohibitively expensive, especially when there are various subdatasets extracted for different analytical purposes. This calls for efficient in-database support of advanced analytical methods. In this paper, we introduce LEADS, a novel SQL-aware dynamic model slicing technique to customize models for specified SQL queries. LEADS improves the predictive modeling of structured data via the mixture of experts (MoE) and maintains efficiency by a SQL-aware gating network. At the core of LEADS is the construction of a general model with multiple expert sub-models trained over the database. The MoE scales up the modeling capacity, enhances effectiveness, and preserves efficiency by activating necessary experts via the SQL-aware gating network during inference. To support in-database analytics, we build an inference extension that integrates LEADS onto PostgreSQL. Our extensive experiments on real-world datasets demonstrate that LEADS consistently outperforms the baseline models, and the in-database inference extension delivers a considerable reduction in inference latency compared to traditional solutions.

==> revision/R5.tex <==
% \begin{table}[]
% \caption{Optimizing UDFs: analyzing the trade-offs between response time and memory usage.}
% \vspace{-1mm}
% \label{tab:udf_memory}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{@{}ccccc@{}}
% \toprule
% Setting  & Workload (20\%) & Workload (40\%) & Workload (80\%) & Workload (100\%) \\ \midrule

% \makecell{INDICES \\ w/ all opt} & 447.72MB/\textbf{6.1s} & 458.97MB/\textbf{12.2s} & 482.23MB/\textbf{24.4s} & 514.42MB/\textbf{30.3s} \\ \midrule

% \makecell{INDICES \\ w/o shared memory}
%   & 460.59MB/13.6s & 481.34MB/27.3s & 512.66MB/54.6s & 528.01MB/68.1s \\ \midrule

% \makecell{INDICES \\ w/o state cache}
%   & \textbf{441.79MB}/82.4s  & \textbf{456.34MB}/164.7s & \textbf{478.19MB}/329.3s &  \textbf{503.93MB}/411.4s \\ 
% \bottomrule
% \end{tabular}%
% }
% \end{table}


\subsection*{Response to Reviewer \#5}
\begin{myquote}
\textbf{W1:} Paper lacks a detailed analysis of computational overheads.

\noindent
\textbf{O1:} The paper introduces several optimization techniques within INDICES, such as efficient execution allocation, memory sharing, and state caching. What are the computational overheads associated with these techniques? It would help to have a detailed analysis with their impact on database performance, memory usage, and query processing times. This needs more analysis to help dbas and system designers better understand the trade-offs involved in implementing INDICES and optimize their systems accordingly.
\end{myquote}
\noindent
\textbf{Response.} 
Efficient execution allocation provides access to high-performance data retrieval APIs, such as the Server Programming Interface (SPI), enabling faster data access. Memory sharing eliminates unnecessary read-write overheads across different execution environments, while state caching reduces the overhead associated with loading and releasing the model for each inference execution.
All three optimization techniques are designed to minimize the response time of the inference query, 
%i.e., SELECT infer(<tableName>, <task>, <propositional formula>) as defined in Section~\ref{sec:workflow}. We experimentally 
for which the effectiveness was validated 
%the effectiveness of these techniques 
in Figure \ref{fig:db_micro}. 

To provide an in-depth analysis of the computational overheads with respect to these optimizations, we conduct a new experiment to investigate the trade-offs between response time and memory usage in the UDF execution process. 
Specifically, we use a workload containing 300 inference queries and record memory usage throughout the entire process. The results are reported in Figure~\ref{fig:udf_memory}. 
We observe that \textit{w/o state caching} has a longer response time for the workload because UDFs need to load models frequently. Additionally, \textit{w/o memory sharing} results in higher time usage compared to \textit{w/ all opts}, due to the repeated copying of data between different execution environments. 
However, memory sharing and model caching do not significantly increase the overall memory cost during the UDF execution process.

% The \Frame equipped with three optimizations significantly reduces time usage while increasing memory usage due to consistently caching the model during the entire workload execution. 
% Conversely, \Frame without state caching dynamically loads the model from disk for each inference and releases the memory allocated to the model, resulting in higher time usage but lower memory usage.

% \bluerevise{
% The \Frame equipped with three optimizations significantly reduces time usage while increasing memory usage due to consistently caching the model during the entire workload execution. 
% Conversely, \Frame without state caching dynamically loads the model from disk for each inference and releases the memory allocated to the model, resulting in higher time usage but lower memory usage. 
% \Frame without memory sharing still benefits from state caching, thus exhibiting lower time usage compared to \Frame without state caching. However, since it does not use shared memory between the Rust and Python execution environments, subdatasets retrieved from Rust are first serialized, copied to the Python environment, and then deserialized. This introduces an extra copy of the retrieved data, leading to the highest memory usage compared to all other settings. Additionally, this data transfer process introduces more overheads and is slower than \Frame equipped with three optimizations.}


We have expanded the description of the three optimization techniques in Section~\ref{subsec:indb_opt} and provided a more comprehensive analysis of the trade-offs between the response time and memory usage in Section~\ref{subsec:RQ3}, with experiment results shown in Figure~\ref{fig:udf_memory}.



\input{revision/complexSQLExample}

\begin{myquote}
\textbf{W2:} Impact of SQL query complexity on the model performance is unclear.

\textbf{O2:} The model slicing approach is dependent on the SQL query's ability to specify relevant sub-data. How does the complexity of SQL queries, including those with multiple nested subqueries or advanced filtering conditions, affect the performance and accuracy of the resulting model? It would be interesting to let users guide users in crafting queries such that the benefits of LEADS are maximized without causing degradation in model performance.
\end{myquote}
\noindent
\textbf{Response.}
We thank the reviewer for this constructive feedback.
We have added new experiments in Section~\ref{subsec:RQ4} to investigate the impact of SQL query complexity on model performance and also assessed the system efficiency when involving JOIN operation in predictive queries.

This study primarily focuses on primitive queries using equality selection predicates, which are conjoined with the logical \texttt{AND} operation, as illustrated in Figure~\ref{fig:SQL}.
The complexity of our supported query is defined by the number of predicates in the \texttt{WHERE} clause. 
In our new experiment, we incrementally added up to 6 predicates to evaluate the prediction results under various query complexity. As shown in Table~\ref{tab:query_complexity_revision}, \Name outperforms baseline methods across different levels of query complexity. Furthermore, we observe an upward trend in predictive performance with the increase in the number of predicates, indicating that complex primitive queries provide more meta-information, enhancing prediction accuracy.

For complex queries, 
%in practical applications, 
\Name cannot directly encode them in inference tasks. 
%As discussed in Section~\ref{sec:encoder}, \Name only supports primitive queries. 
However, we can still apply \Name 
%in complex queries 
by rewriting them to primitive queries. 
For example, for queries with predicates conjoined by the \texttt{OR} operation, we can split them into several primitive queries for independent inference, as shown in Figure~\ref{revisefig:query_or}. 
%\Name cannot directly support multiple nested queries either. Instead, 
For nested queries, we can execute the inner query first to get intermediate results, then rewrite the out query as primitive queries and conduct inference, as shown in Figure~\ref{revisefig:query_nested}.


\ignore{
In this study, we primarily focus on primitive queries that use equality selection predicates, which are conjoined using the logical AND operation, as illustrated in Figure~\ref{fig:UnitSQL}.
For complicated queries that can be rewritten into primitive queries with multiple equality selection predicates, our LEADS delivers high performance. This is experimentally validated in Table~\ref{tab:mainstudy}. 
%% wyc: the answer seems not straightforward enough, what about those queries with nested subqueries? 

\red{TODO: straightly answer to multiple nested subqueries or advanced filtering conditions. Query Complexity -> Number of predication. (No need to keep the predictive data same)}

Therefore, complex queries within our supported query types are those with more random predicates.
LEADS relies on a gating network to dynamically generate meta-information based on the filter conditions in an SQL query, which customizes the general model for a specified subdataset. This customized model enhances inference effectiveness while maintaining efficiency. Consequently, queries with more predicates tend to generate more meta-information and lead to more accurate predictions for their corresponding subdataset, as illustrated in Figure~\ref{fig:sqlgate_ablation}. 
In this figure, the red bar represents the model's performance without meta-information, which is lower than the performance depicted by the blue bar with meta-information.
}







==> revision/R6.tex <==

\subsection*{Response to Reviewer \#6}
\begin{myquote}
\noindent
\textbf{W1:} It seems that the two contributions (MOE and In-database inference) do not have close relationship.
\end{myquote}
\noindent
\textbf{Response.} 
We would like to clarify that our objective is to build an end-to-end in-database inference system INDICES that supports SQL-aware predictive modeling. 
%
Both MoE and in-database inference are integral components in INDICES. 
Specifically, we build a general model based on the Mixture-of-Experts (MoE) technique at the training stage. The experts in the model are trained to specialize in different problem subspaces for more effective predictive modeling. 
Then, when a SQL query comes at the inference stage, our in-database inference component will load the trained model and slice a subset of the experts (aka. sliced model) from it based on the query conditions for prediction.
The MoE component helps this sliced model achieve higher inference accuracy for specific SQL queries, while the in-database inference component ensures faster model inference execution. Together, these two contributions support our end-to-end system INDICES.

%in the training and inference stages of the predictive modeling, as shown in Figure~\ref{fig:system}.}
%% wyc: may highlight that MoE and inference emphasize two stages of the workflow in Figure 5 (to justify that they are related in some way). The following only re-iterate the two components separately. 
%Specifically, we introduce a novel LEADS technique based on the Mixture-of-Experts (MoE) technique to enhance effectiveness.
%To mitigate the additional computational cost from MoE, we propose a SQL-aware gating network in \Name which dynamically activates a few experts specified by SQL queries to keep the inference efficient.
%Second, we have integrated the \Name technique into PostgreSQL as a plug-in extension and applied three optimizations to reduce execution overheads further and speed up the inference time. 

We have added more explanations in Section~\ref{sec:introduction} to clarify the relationship between the MoE and in-database inference components in our INDICES system. 

% \red{TODO:directly connect these two contributions}


\begin{myquote}
\noindent
\textbf{W2:} Why not compare with existing works (e.g., the second part in related work) to demonstrate the efficiency of in-database inference?
\end{myquote}
\noindent
\textbf{Response.} 
MADlib\cite{hellerstein2012madlib} only supports feeding the static model with tuples in a data table and does not adaptively feed the model with meta-information such as query encoding to dynamically customize the model for inference as our system does. 
% \red{Adding this support is non-trivial and requires significant changes to the MADlib infrastructure.}
Google ML library\cite{GoogleML} and Microsoft’s SQL Server Machine Learning Services\cite{microsoft} 
share similar limitations. 
Additionally, they only make their service public while the infrastructure code is not accessible.
Therefore, none of them are directly comparable.
\cite{xingNAS} primarily integrates the model selection process into PostgreSQL for advanced data analysis, which is a step before model inference and orthogonal to our work, making it incomparable.
We have explained the distinctive objectives and designs between our work and existing works
in Section~\ref{sec:relatedWork}.



\begin{myquote}
\noindent
\textbf{W3:} It seems that the paper does not consider the data distribution in database. If the data updates, given the same SQL, will the output be same? Is that reasonable?
\end{myquote}
\noindent
\textbf{Response.} 
We would like to clarify that the model is trained with the workloads generated by Algorithm~\ref{alg:create_workload} under the assumption that both training and testing data are drawn independently from the same distribution, i.e., the Independent and Identically Distributed (i.i.d.) assumption.

We have added experiments to evaluate the effectiveness of the \Name technique in scenarios where the same SQL queries are executed twice with data changes between the two snapshots. 
In these cases, the SQL query encoding remains the same, but the selected subdatasets may differ.
Specifically, we use the Credit and Diabetes datasets and employ a DNN as the base model.
Each dataset is divided into two parts: the first part represents the original data stored in the database while the second part consists of new data to be inserted.
The new data are sequentially inserted into the database as five sets of insertions, and the model is evaluated on the same SQL queries after each set of insertions using the metrics Workload-AUC.
Figure \ref{fig:insertion_workload_auc} illustrates that 
although the selected subdatasets differ due to the new data, the model enhanced by the \Name technique continues to perform effective inference on these subdatasets and consistently outperforms the base model (without the \Name enhancement).

In summary, as long as the updated data continues to follow the i.i.d. assumption, our trained model, enhanced by \Name, can generalize well to predict new data.
We have added the experimental results and corresponding analysis in Section~\ref{subsec:RQ4}.


% \begin{figure}[t]
% \centering
% % \captionsetup{justification=centering}
% \begin{subfigure}[b]{0.49\textwidth}
%     \hspace{2mm}
%     \centering
%     \includegraphics[width=0.45\columnwidth]{figs/revision/insertion_legend.pdf}
% \end{subfigure}

% \begin{subfigure}[b]{0.24\textwidth}
%     \centering
%     \captionsetup{justification=centering,margin={0cm,0.7cm}}
%     \includegraphics[width=0.99\columnwidth]{figs/revision/credit_workload_auc.pdf}
%         \caption{Credit}
% \end{subfigure}
% ~
% \begin{subfigure}[b]{0.24\textwidth}
%     \centering
%     \captionsetup{justification=centering,,margin={0cm,0.7cm}}
%     \includegraphics[width=0.99\columnwidth]{figs/revision/diabetes_workload_auc.pdf}
%     \caption{Diabetes}
% \end{subfigure}
% \caption{Effects of data insertion on Workload-AUC.}
% \vspace{0mm}
% \label{revise:insertion_workload}
% \end{figure}


% \begin{figure}[t]
% \centering
% \begin{subfigure}[b]{0.49\textwidth}
%     \hspace{1mm}
%     \centering    \includegraphics[width=0.75\columnwidth]{figs/db/spj_legend.pdf}
% \end{subfigure}

% \begin{subfigure}[b]{0.24\textwidth}
%     \centering
%     \includegraphics[width=0.95\columnwidth]{figs/revision/macro_join.pdf}
%         \caption{Response time comparison for SPJ and Non-SPJ queries.}
%             \label{revisefig:spj}
% \end{subfigure}
% ~
% \begin{subfigure}[b]{0.24\textwidth}
%     \centering
%     \includegraphics[width=0.95\columnwidth]
%     {figs/revision/sql_2.pdf}
%     \caption{Example for SPJ (red box) and Non-SPJ queries (blue box).}
%     \label{revisefig:spj_example}
% \end{subfigure}
% \caption{Efficiency evaluation of \Frame for SPJ queries.  \Frame-decoupled (I-d) and \Frame (I) approaches.  
% }
% \end{figure}

\begin{myquote}
\noindent
\textbf{W4:} It seems that the paper just considers equality selection in SQLs, but in general, SPJ queries should be supported.
\end{myquote}
\noindent
\textbf{Response.} 
In this study, we primarily focus on primitive queries that use equality selection predicates, which are conjoined using the logical AND operation, as illustrated in Figure~\ref{fig:UnitSQL}. 

We have conducted a new experiment to verify the efficiency of \Frame in executing SPJ queries in Section~\ref{subsec:RQ4}.
In this experiment, we involve a JOIN operation in the inference query. Specifically, we first join two tables to form the entire dataset and retrieve the predictive subdataset corresponding to the query, as illustrated in the example SQL in Figure~\ref{fig:spj_example}.
The results, shown in Figure~\ref{fig:spj}, indicate that \Frame still outperforms the baseline method (INDICES-decouple) due to the reduced overhead of moving data out of the database. For further comparison, we execute the simple query, referred to as Non-SPJ queries, with the same filter conditions without a JOIN operation. We notice that for queries with JOIN operations, the speedup of \Frame compared to the baseline is not as significant as for Non-SPJ queries. This is because, for complex join queries, the benefit of eliminating network latency is less pronounced. The longer query planning and execution times dominate the overall query time.
Additionally, our \Name technique only encodes the filter conditions in the SELECT query, so the JOIN operation does not directly impact the effectiveness of our system.

Therefore, we would like to clarify that our system \Frame can easily support SPJ queries.



\begin{myquote}
\noindent
\textbf{W5:} How to deal with schema change in the proposed framework.
\end{myquote}
\noindent
\textbf{Response.} 
If the schema changes due to the insertion or deletion of columns in the predictive table, the dimension of the data feature vector will change, leading to a dimension mismatch between the data feature vector and the well-trained model. Thus, the model needs to be retrained from scratch to adapt to the latest feature space of both SQL feature vectors and data feature vectors.

However, if we want to continue using the original models to serve inference, we have different solutions for attribute insertion and deletion.
For attribute insertion, the database retains the original data. Using the PROJECTION operation, we can fetch tuples with specific attributes and feed them to the model for inference. However, the newly added attributes will not be considered in the predictive modeling.
For attribute deletion, values in the deleted attribute will be missing. We pad these missing values with a special token or the most frequent token to form a fixed dimension input for inference, which leads to a degradation of prediction accuracy. Experiments are conducted to investigate the effect of attribute deletion on effectiveness. The results, shown in Figure~\ref{fig:schema_change}, indicate that as the number of deleted attributes increases, the performance of the model decreases. We also notice that in the Credit dataset, the Workload-AUC collapses when the number of deleted attributes increases from 8 to 16, while in the Diabetes dataset, a significant reduction occurs when deleting the first attribute. This suggests that the importance of attributes varies, and their deletions have different effects on prediction results.

In summary, while temporary solutions for schema changes exist, they lead to performance degradation or the neglect of new attributes. Therefore, retraining the model is the recommended approach to ensure predictive accuracy. We have added a discussion about schema change in Section~\ref{subsec:RQ4}.

% However, if we still 
% \red{TODO: We have added the description of handling schema change in "Assumptions" of Section~\ref{sec:preliminaries}.}

\begin{myquote}
\noindent
\textbf{W6:} It would be better to make Algorithm 1 closer to the corresponding citations for better clarity.
\end{myquote}
\noindent
\textbf{Response.} 
As suggested, we have moved Algorithm~\ref{alg:create_workload} to Section~\ref{subsubsec:workload} where we first introduce it for better clarity.



==> revision/R7.tex <==


\subsection*{Response to Reviewer \#7}
\begin{myquote}
\textbf{W1:} The motivation of the SQL-aware structured data analytics problem needs more justifications.

\noindent
\textbf{D1:} First of all, the motivation of the new problem is not well justified. The example in Figure 1 is too ambiguous. It mentions the task of "evaluating the influence of education and city location on the incomes of different subdatasets". However, there is little information about why in-database ML is needed and what is the real application scenario of such a task. As a result, the significance of the new problem is not clearly illustrated.
\end{myquote}
\noindent
\textbf{Response.} 
As suggested, we have added more justifications to better motivate our SQL-aware predictive modeling problem and in-database ML in Section~\ref{sec:introduction} and Section~\ref{sec:preliminaries}. Moreover, we have refined Figure 1 to make the example clearer.
%further justified the motivations for in-database ML and SQL-aware predictive modeling in Section~\ref{sec:introduction} and Section~\ref{sec:preliminaries}, respectively. In the meantime, we have modified Figure 1 to better illustrate the motivation.

First, 
%for SQL-aware predictive modeling, we note that 
%(1) We would like to clarify the motivation behind the SQL-aware predictive modeling. 
we note that data analysts are often interested in performing analytics on specific subsets of data. 
For example, in healthcare applications, doctors may want to assess the readmission rates among patients diagnosed with a particular disease, while in e-commerce applications, marketing analysts may want to analyze the click-through rate (CTR) within a specific age group. 
Naturally, they prefer effective models that capture fine-grained patterns within these subdatasets. 
Unfortunately, the general model trained on the entire dataset may not be effective for subdatasets, while training separate models for each subdataset is computationally prohibitive due to the huge number of possible combinations. 
Therefore, we formulate our SQL-aware predictive modeling problem considering the need for this kind of analysis. 
%to seek solutions for the analysis requirement.

Second, we would like to clarify that in-database ML allows analysts to define their analytical tasks using SQL query and perform computations within the database directly, without the need for moving data to an external ML platform.
It is not only user-friendly to analysts, but also mitigates the potential issues caused by data movement, e.g., time-consuming, error-prone, or even impossible due to privacy and compliance concerns~\cite{abo2018database,hellerstein2012madlib,feng2012towards,zhang2021distributed, yang2022optimizing, xu2022database}. 

Third, 
%% wyc: may combine the third point with the second
we use income prediction as our example because it is a popular task in structured data analysis, which enables informed financial decisions and personalized service offerings \cite{census_source}. In real applications, \cite{GoogleMLApp} proposes predicting income based on attributes such as age, education level, and occupation.
We have included more explanations regarding Figure 1 in the revised paper. 




\begin{myquote}
\textbf{W2:} The experiment setup is insufficient to support the proposed new problem.

\noindent
\textbf{D2:} In addition to that, the experiment setup is problematic. Even if we assume that the new problem is important in some kinds of real applications, the authors did not provide enough evidence in the choice of datasets and workloads: the datasets are too small and could just be stored in .csv files and directly apply the Python based ML libs. Meanwhile, the SQL clauses are synthetic and with very simple structures. To sum up, it does not provide enough evidence to show that (i) the scale of the datasets is large enough that needs in-database ML; (ii) the SQL clauses are complicated enough that lead to significant research challenges.
\end{myquote}
\noindent
\textbf{Response.} 
% (1) We have added a large dataset, Avazu, which has an order of magnitude increase in the number of data items and features
% \red{TODO:directly mention the numbers} 
% compared to previous datasets. The detailed profile of Avazu is presented in Section~\ref{subsec:expSetup} and Table~\ref{tab:dataset}. 
We thank the reviewer for this constructive comment. 
We have added new experiments with a much larger dataset and with more complicated SQL queries in Section~\ref{sec:experiment}. The results further confirm the effectiveness and efficiency of our technique. We provide more details below.

First, we have added a new dataset, Avazu~\cite{avazu}, which consists of 40,428,967 tuples and 1,544,250 features. 
%as illustrated in Section~\ref{subsec:expSetup} and Table~\ref{tab:dataset}.
We conducted two sets of experiments on Avazu to verify the effectiveness of \Name and the efficiency of INDICES, as presented in Table~\ref{tab:mainstudy} and Figure~\ref{fig:db_macro}, respectively. 
We observe in Table~\ref{tab:mainstudy} that \Name outperforms the four base models in terms of AUC on the Avazu dataset. 
%% wyc: \red{better show some numbers here.}
Similarly, in the efficiency experiment in Figure~\ref{fig:db_macro}, INDICES also significantly reduces the end-to-end response time compared to the INDICES-decoupled baseline on this dataset. 
The results are consistent with those on other datasets, demonstrating that our techniques can handle large-scale datasets well.
%% wyc: need double check whether there is any difference between this large dataset and smaller datasets. 


%First, we experiment on Avazu to verify the effectiveness of \Name. The results in Table~\ref{tab:mainstudy} demonstrate that \Name technique improves the AUC across four base models on the Avazu dataset. 
%In the efficiency experiment in Figure~\ref{fig:db_macro}, we keep the number of predictive records the same between datasets for fairness as described in Section~\ref{subsec:RQ3}.
%we compare the response time of INDICES on the Avazu dataset and notice that INDICES significantly reduces the end-to-end response time compared to the INDICES-decoupled baseline. Therefore, we declare that our \Name technique and \Frame can handle large-scale datasets well. 
%In addition, we have emphasized the importance of in-database inference in Section~\ref{sec:introduction} and Section~\ref{sec:indb_inference}. Compared to using CSV files directly, the key benefit is that data does not need to be moved out of the database. This approach ensures data privacy and security based on the authentication mechanism of the database and eliminates the cost of data transfer to speed up the inference process.
%% wyc: the benefit of using in-database ML is already replied in the previous response, here his main concern is the small dataset, so may not need to repeat it
\ignore{
Second, we would like to clarify our main research challenge is how to utilize the meta-information provided in SQL queries to customize the predictive model and achieve better performance on retrieved subdatasets.
Then, as for the SQL queries, we primarily focus on primitive queries that use equality selection predicates, conjoined using the logical \textit{AND} operation, as illustrated in Section~\ref{sec:encoder}. The complexity of SQL varies with the randomness of the number of predicates and their values. Training a general model once and dynamically slicing the model based on all possible queries is a challenging problem proposed in our work. We formalize it in Section~\ref{sec:preliminaries}, propose our solution \Name in Section~\ref{sec:sql_aware_network} and empirically evaluate \Name in Section~\ref{sec:experiment}.
\red{The second point seems only explain what have already presented in the original paper. It may not be sufficient as this comment is questioning the experiment. Would it be better to mention the new results with complicated SPJ queries here to strengthen the response?}}

Second, \Name currently only accepts the input in the form of \texttt{primitive queries}, which use equality selection predicates conjoined with the logical \texttt{AND} operation, as illustrated in Section~\ref{sec:encoder}. 
%The complexity of SQL queries varies with the randomness of the number of predicates and their values. We have added a new experiment to investigate the impact of the number of predicates on the model prediction, with result shown in Table~\ref{tab:query_complexity}. 
For more complicated queries, such as those with $OR$ operations and multiple nested queries, we can rewrite them into primitive queries and apply \Name for inference tasks. Please refer to Figure~\ref{revisefig:query} for two rewriting examples. 
Moreover, our \Frame supports SJP (Select-Project-Join) queries, which incorporate the \texttt{JOIN} operation. We have added a new experiment to evaluate the efficiency of \Name on SPJ queries, as shown in Figure~\ref{fig:spj}. The results demonstrate that our system can process SPJ queries efficiently.
%In summary, \Name can model all possible primitive queries with varying numbers of predicates and can be easily extended to handle many practical complex queries.


\ignore{
(1) We have added an experiment to evaluate the performance of our in-database inference system on the large Avazu dataset, summarized in Table~\ref{tab:dataset} and Section~\ref{subsec:expSetup}. Avazu has an order of magnitude increase in both the number of data items and the number of features, compared with previous datasets. The results in Table~\ref{tab:mainstudy} demonstrate that our system, enhanced with LEADS, can effectively improve the AUC across four base models on the Avazu dataset.

In addition, we have further emphasized the importance of in-database inference in Section~\ref{sec:introduction} and Section~\ref{sec:indb_inference}. 
Specifically, in-database inference offers two key benefits. First, users can issue various SQL queries with different predicates to select subdatasets for prediction. With an advanced query optimizer in the database, only the selected subdataset is kept in memory for further processing. In contrast, using CSV files requires loading all data into memory before selecting the corresponding subdatasets.
Second, as illustrated in Figure\ref{fig:db_scalability}, our in-database inference system significantly reduces the end-to-end response time compared to the INDICES-decoupled baseline, across datasets ranging from 40k to 640k tuples. The INDICES-decoupled baseline involves loading the entire dataset from the database into an external service that uses Python-based ML libraries.

(2) We would like to clarify that the main research challenge addressed in this study is how to efficiently train models for effective predictive modeling across analyst-specified subdatasets.
Specifically, we primarily focus on primitive queries that use equality selection predicates, conjoined using the logical AND operation, as illustrated in Section~\ref{subsec:SQLQueryModel}. The complexity of SQL varies with the randomness of the number of predicates and their values. Training a general model once and dynamically slicing the model based on any dynamic query is a challenging problem yet to be solved. In this paper, we propose a novel LEADS technique to effectively address this problem, as discussed in "Problem Formulation" Section~\ref{sec:preliminaries} and empirically evaluated in Section~\ref{sec:experiment}.}




\begin{myquote}
\textbf{D3:} Following the above item, a case study of real-world application is needed in addition to current results of effectiveness.
\end{myquote}
\noindent
\textbf{Response.} 
%\bluerevise{We agree that a case study of real-world application would add value to the experimental evaluation. }
%
As suggested, we have added more detailed descriptions to our case study on the Diabetes dataset in Section~\ref{subsec:RQ1} and the result is shown in Figure~\ref{fig:worst_sql_compare}.

In the Diabetes dataset, we predict the readmission rate for patients based on medications and laboratory results. This helps hospitals or healthcare providers identify high-risk patients, improve care, and reduce readmissions in real-life applications. We investigate the top-4 SQL queries that result in the most significant performance improvement from \Name. 
We found that these queries retrieve only a small amount of data from the training dataset. Insufficient supervised data prevents the training model from fully capturing patterns in this subdataset, leading to poorer inference performance. 
However, Figure~\ref{fig:worst_sql_compare} demonstrates that our LEADS technique can effectively mitigate this performance collapse, where the sliced model can capture the more fine-grained patterns within subdatasets, due to the assistance of meta-information from SQL queries.



\begin{myquote}
\textbf{D4:} The efforts in Section 5 is more like engineering practice rather than research contribution. Also from the code repo provided by the authors, it seems that the authors just did some simulations rather than integrating the proposed framework with the core of DBMS. Thus the technical contribution of Section 5 might not be so convincing.
\end{myquote}
\noindent
\textbf{Response.} 
We would like to clarify that our main objective is to build an efficient in-database inference system, where the research challenge from the system perspective is how to improve the efficiency of inference execution for subdatasets queried from the RDBMS~\cite{yesql}.
%
To address such a challenge, we propose three optimization techniques to efficiently integrate the inference process into the RDBMS via UDF. 
%as shown in Figure~\ref{fig:udf} and illustrated in Section~\ref{subsec:indb_opt}.
We validate in Section~\ref{subsec:RQ3} that these optimizations significantly outperforms the decoupled database and inference server approach in terms of response time.
%Additionally, Section~\ref{sec:workflow} introduces the SQL interface, training data collection, and the end-to-end pipeline from training to inference execution, which is core to adopting our system in real usage.

As for our implementation, we integrate the proposed LEADS 
technique into PostgreSQL via an extension developed based on pgrx\footnote{\url{https://github.com/NLGithubWP/indices/tree/main/internal/pg_extension}}, enabling model inference with a single SQL statement:
SELECT infer(<tableName>, <task>, <propositional formula>).
We used PostgreSQL 14 in our experiments. %We have added the PostgreSQL version in Section~\ref{sec:experiment}.
%The experiment in Section~\ref{subsec:RQ3} reports the response time of the whole inference SQL execution.



\begin{myquote}
\textbf{D5:} The survey of related works in Section 7 is not detailed enough. Besides, I believe the term of in-database ML should refer to works that tried to use relational operators to express the ML models, such as "Learning Linear Regression Models over Factorized Joins. SIGMOD 2016". The efforts made in this submission with UDF is not making the similar level of efforts with in-database ML works and the position of this submission should be further clarified when introducing related works.
\end{myquote}
\noindent
\textbf{Response.}
As suggested, we have added more related works with respect to MoE and in-database machine learning in Section~\ref{sec:relatedWork}.
%Briefly, we add a discussion about the background of MoE and point out the difference between our work and previous works. Also, we have added the related work on in-database machine learning, presented the distinctions, and explained the differences between our proposal and existing works.

We agree that expressing ML models with relational operators as done in \cite{schleich2016learning} requires a lot of efforts. 
However, 
%this kind of 
such a technique only supports feeding the static model with tuples in a table, and it is non-trivial to extend its support to complex machine learning models. Furthermore, it cannot customize the model for inference with meta-information such as query encoding.
%Instead of focusing on simple linear regression models as in
%\cite{schleich2016learning}, 
%% wyc: is there any other work similar to this reference?
In this paper, we target complex deep learning models which have been recognized as a more effective approach for structured data analysis. 
%The core component of our system is a novel SQL-aware dynamic model-slicing technique called LEADS, which is a model-agnostic enhancement technique for deep learning models in SQL-aware predictive modeling. 
%Compared with \cite{schleich2016learning}, our work makes significant and novel contributions in two main areas. First, we formalize a new problem that involves retrieving queries rather than simple predictive tasks.
%Second, we propose the \Name technique, which enhances deep learning models to address the problem.
%% wyc: the above novel contributions can be answered in below responses, here better emphasize the differences.
%
Therefore, we choose to integrate ML into the database via UDF, which enables seamless integration with existing RDBMS and is highly extensible. 
%and enhances their analytics capability \cite{hellerstein2012madlib}. 
We further propose three optimization techniques in our system to efficiently execute model inference with UDF. 
%The key research challenge is how to efficiently execute the proposed algorithm in UDF \cite{yesql}. 
%Our work proposes three optimization techniques to improve inference efficiency, which are detailed in Section 5.1 and empirically verified in Section 6.4.
We have also clarified the differences between our work and these works in Section~\ref{sec:relatedWork}.


\begin{myquote}
\textbf{W3:} Some claims needed to be adjusted or explained.\\
\textbf{D6:} The claims of the contribution in the introduction should be accurate. The claim "this is the first work that develops techniques and a system to address the problem" is too ambiguous and fails to properly describe the significance of this work. Also the terms like "scales up the modeling capacity" and "advanced structured data analytics" are too general and didn't provide enough insights.
\end{myquote}
\noindent
\textbf{Response.} 
%As suggested, we have further explained the contributions in the introduction (Section~\ref{sec:introduction}) and added descriptions for the claims mentioned in this comment.
%% 
We have revised the presentation in Section~\ref{sec:introduction} to make the claims more accurate. Regarding the claim: "this is the first work that develops techniques and a system to address the problem", we have double-checked related works and ensured that this claim is correct. We have also included more explanations in Section~\ref{sec:introduction} to clarify the significance of our work and support this claim.

%We would like to clarify the significance of our work explicitly. 
%Our work introduces the LEAD technique, which involves training a single general model and dynamically slicing it based on SQL queries during inference. 
%This method effectively addresses the analytics task on subdatasets specified by certain queries, which are formalized as SQL-aware predictive modeling in Section~\ref{sec:preliminaries}. 
%Furthermore, we develop an in-database inference system that integrates the LEADS technique into the Postgres database, complemented by three optimization techniques to enhance inference efficiency.
%To the best of our knowledge, we are not aware of any existing work or system that addresses the same issues and provides the same functionality.



\begin{myquote}
\textbf{D7:} The novelty of the proposed framework needs justification. A large portion of the technical contribution is to leverage the MoE model. However, the efforts made in Section 4 could just be summarized it to adopt the MoE model to structural data classification/regression. And there is no significant technical challenges brought by the SQL clauses since the slicing is mainly done according to the WHERE predicates. If the authors could show a case with more complicated queries such as those with join operation between multiple tables or conjunctions, the technical contribution could be more convincing.
\end{myquote}
\noindent
\textbf{Response.} 
As advised, we have added more justifications in Section~\ref{sec:introduction}, Section~\ref{sec:sql_aware_network}, and Section~\ref{sec:indb_inference} to clarify the novelty of our proposed framework.  
%(1) We would like to summarize our technical contributions and novelty as follows: 
Specifically, there are three main technical contributions:
%
(a) We are the first to formulate and identify the challenges of SQL-aware predictive modeling in structured data analytics, specifically, making predictions on a selected subset of tuples from logical tables.
%
(b) We propose a novel technique, called LEADS, to address the problem, which harnesses the meta-information provided in SQL queries to customize the model for better predictive performance on the retrieved subdataset.
% in short for LEADS
(c) We build an end-to-end system, called INDICES, which incorporates three optimization techniques to speed up the in-database inference: the utilization of SPI, shared memory, and state caching.

% LEADS. MoE
We  would like to further clarify our efforts in adopting the MOE model for structured data as follows:
(a) We develop the SQL-aware gating network that generates expert weight based on embeddings of SQL queries instead of input data. These embeddings carry meta-information about shared attributes in the predictive data, facilitating the expert selection in inference.
(b) The learnable sparsemax function is applied in the final layer of the SQL-aware gating network to generate sparser scores. Compared to normal softmax, it reduces the number of activated experts and improves the inference speed. The benefits of sparsemax are illustrated in Section~\ref{sec:preliminaries} and proven in the ablation study in Figure~\ref{fig:exp_sparsemax_auc}.
(c) We propose two regularization terms in Section~\ref{sec:optimization}. 
The balance term ensures each expert is fully trained and keeps the stability of the training process. 
The sparse term minimizes the number of selected experts, further speeding up inference. The impact of regularization terms is demonstrated in Figure~\ref{fig:exp_reg_auc} and Figure~\ref{fig:exp_reg_expert_frequency}.

Moreover, we focus on the WHERE clause in SQL queries because the filter conditions provide the profile of predictive data. Handling the diverse combinations of predicates and logical operators within the WHERE clause presents a notable technical challenge in modeling, as detailed in Section~\ref{sec:encoder}.
Additionally, our approach can handle more complicated queries with INDICES, such as the JOIN and PROJECTION operations. 
We have added new experiments with respect to SPJ queries in Section~\ref{subsec:RQ4}.
The results depicted in Figure~\ref{fig:spj} demonstrate that our system processes SPJ queries faster than the baseline.

% \balance

==> revision/complexSQLExample.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.24\textwidth}

    \centering
    \captionsetup{justification=centering,margin={0cm,0cm}}
    \includegraphics[width=0.95\columnwidth]{figs/revision/OR_REWRITE.pdf}
        \caption{Handling query with \texttt{OR} operation}
          \label{revisefig:query_or}
\end{subfigure}
~
\begin{subfigure}[b]{0.24\textwidth}

    \centering
    \captionsetup{justification=centering,,margin={0cm,0cm}}
    \includegraphics[width=0.95\columnwidth]{figs/revision/NESTED_REWRITE.pdf}

    \caption{Handling query with nested conditions}
            \label{revisefig:query_nested}
\end{subfigure}
\caption{Examples of handling complex SQL query}
\vspace{3mm}
\label{revisefig:query}
\end{figure}

==> revision/revision.tex <==
\pagestyle{empty}
\thispagestyle{plain}

\twocolumn


% \centerline{\textbf{Steps in checking the revised paper}}
% \vspace{10mm}

% Logic
% \red{
% NL: Now check this

% \textbf{Steps in checking the revised paper:}
% \begin{itemize}
%     \item Figures, Sections References.
%     \item Each point is answered, and marked in blue in the main script.
%     \item Consistent description.
%     \item Grammarly
%     \item Summary of change includes this
%     \item Use "design" and "propose"
% \end{itemize}


% \centerline{\textbf{Response Logic}}
% \vspace{5mm}

% \begin{itemize}
%     \item A. \red{Optionally thank the reviewer (no need to thank everywhere)}
%     \item B. Answer \red{directly} to the question/requirement of the reviewer
%     \item C. Provide details of new results/discussion/figures/tables and etc in the response,
%     \item D. Update and highlight the manuscript to address the concern.
%     \item E. \red{state how and where you have addressed the concern.} \\ 
%     E.1 We have done what in where ... \\ 
%     E.2 long sentence + new paragraph
% \end{itemize}
% }

\noindent \textbf{\Large Response to Reviewers' Comments}
\vspace{5mm}

\noindent 
We would like to thank the meta-reviewer and all the reviewers for their insightful and constructive comments.
We have carefully addressed the comments and revised the manuscript, where major changes are highlighted in {\color{blue} blue}.
In what follows, we first summarize the major changes that we have made and then provide a point-by-point response to each reviewer's comments.


% nl: this follows the sequence of the meta-reviewer's question.
\subsection*{Summary of Changes}
\begin{itemize}[leftmargin=*]
    \item We have clarified the novelty of the SQL-aware model slicing (LEADS) technique and the motivation to implement an inference system (INDICES) with LEADS on the Postgres in Section~\ref{sec:introduction}.
    % \item We have made the motivation example in Figure~\ref{fig:motivation} more
    %\item We have added a formal definition of the SQL-aware predictive modeling problem, given a detailed assumption for our work, and added the formal discussion about the structure data in Section~\ref{sec:preliminaries}.
    \item We have included a description of the structured data and added a formal definition of the SQL-aware predictive modeling in Section~\ref{sec:preliminaries}.
    \item We have added a brief description of the motivation of the LEADS technique and introduced the effect of each component in LEADS for solving the SQL-aware predictive modeling in structure data analytics in Section~\ref{sec:sql_aware_network}.
    \item We have clarified our contributions in implementing  INDICES and added more descriptions about the three optimizations for efficient inference in Section~\ref{sec:indb_inference}.
    \item We have added a new dataset (Avazu) in Section~\ref{subsec:expSetup} to evaluate the effectiveness of our LEADS technique on a larger dataset. The dataset statistics and experimental results are updated in Table~\ref{tab:dataset} and Table~\ref{tab:mainstudy} respectively.
    \item We have included a discussion on the complexity of our supported SQL queries in  Section~\ref{subsec:RQ1} and conducted experiments to analyze the impact of the number of predicates on predictive results.
    \item We have added an in-depth analysis of the trade-offs between the response time and memory usage in Section~\ref{subsec:RQ3}, with results shown in Figure~\ref{fig:udf_memory}.
    \item  We have conducted a new study to evaluate the performance of the \Frame system in complex inference scenarios, specifically focusing on data updates, schema changes, and Select-Join-Projection (SPJ) queries. The experimental results are presented in Figure~\ref{fig:insertion_workload_auc} and Figure~\ref{fig:spj}, with detailed descriptions provided in Section~\ref{subsec:RQ4}.
    \item Finally, we have added more related works and discussions on Mixture-of-Experts and in-database machine learning inference systems in Section~\ref{sec:relatedWork}. % and explained why some related in-database inference systems are not considered as baselines in our experimental study in Section~\ref{sec:relatedWork}.
    \ignore{\item To make space for the above changes, we have shortened ... and extended ... of the original paper. 
    We instead refer the readers to our online technical report 1 for this information.}
    
\end{itemize}

\subsection*{Response to Meta-Reviewer}
\begin{myquote}
\textbf{Comment 1:} The effectiveness/contribution of the proposed method needs more justification (R\#5.o1-o2, R\#6.W2-W3, R\#7.D1, D3-D4, D6-D7).
\end{myquote}

\noindent
\textbf{Response.}
As suggested, we have added more justifications regarding the effectiveness and contributions of our proposed method. 
First, we have added more explanations about the contributions of our proposed system, INDICES, and its core technique, LEADS, in Section~\ref{sec:introduction}, and also included a real-world example of in-database inference in Figure~\ref{fig:motivation} (R\#7.D1, D3, D6, D7). 
Second, for \Name technique, we 
detailed the challenges and our contributions when adopting MoE techniques in Section~\ref{sec:sql_aware_network}. 
Third, for \Frame system, we provided the details of implementation and system-level challenges in Section~\ref{sec:indb_inference}.
Then, we have added new experiments to demonstrate the effectiveness of our method, including an in-depth analysis of the trade-offs between memory usage and response time (R\#5.O1) in Figure~\ref{fig:udf_memory}, the investigation for the complexity of primitive queries shown in Table~\ref{tab:query_complexity_revision} (R\#5.O2), 
adding a larger dataset (Avazu) in Section~\ref{subsec:RQ1}, empirical demonstration of performance on SPJ queries, and performance changes with data updates and schema changes (R\#6.W3) in Section~\ref{subsec:RQ4}. 

Please refer to our responses to R\#5.o1-o2, R\#6.W2-W3, R\#7.D1, D3-D4, D6-D7 below for further details.



\begin{myquote}
\textbf{Comment 2:} It seems the authors overclaim their contributions in many cases (as pointed out in R\#7.D4, D6 and D7). It is required to fix certain claims and add some discussions about the more general cases like the issues mentioned in R\#7.D2.
\end{myquote}

\noindent
\textbf{Response.}
To appropriately describe our contributions to our system INDICES and its core technique LEADS, we first justified the motivation for the in-database inference system and the novelty of the LEADS technique by discussing the challenge in adopting MoE in Section~\ref{sec:introduction}. (R\#7.D6, D7)
Then, we added more detailed discussions about our proposed optimizations in implementations of INDICES in Section~\ref{sec:indb_inference} as our technical contribution. (R\#7.D4)

In addition, we have added more discussion about the workload generation and data choices in Section~\ref{subsec:expSetup} and have included additional experiments to demonstrate the performance of our INDICES system and the effectiveness of the LEADS technique. These include an evaluation of the effectiveness of our system on a large Avazu dataset (Table~\ref{tab:mainstudy}) and an evaluation of the efficiency of our system on SPJ queries (Figure~\ref{fig:spj}). (R\#7.D2)

Please refer to our responses to R\#7.D4, D6, D7, and D2 below for further details.


\begin{myquote}
\textbf{Comment 3:} The presentation need to be further improved (R\#6.W1, W6, R\#7.D5).
\end{myquote}


\noindent
\textbf{Response.}
In the revised manuscript, we have significantly enhanced our paper in terms of presentation and structure. 
Specifically, we have clarified the connection between our proposed LEADS technique and system optimizations in Section~\ref{sec:introduction},
reorganized the preliminary and problem formulation parts to make clear the problem in Section~\ref{sec:preliminaries} (R\#6.W1),
moved Algorithm 1 from Section ~\ref{sec:indb_inference} of the original paper to Section~\ref{subsec:expSetup} (R\#6.W6), added more related work to Section~\ref{sec:relatedWork}, and emphasized our main contributions in Section~\ref{sec:introduction} (R\#7.D5).

Please refer to our responses to R\#6.W1, R\#6.W6, and R\#7.D5 for more details.

\begin{myquote}
\textbf{Comment 4:} The experiments are missing some important elements, including more comparisons with relevant works (R\#6.W2, W6, R\#7.D5), and the incorporation of additional and reasonable experimental settings (R\#6.W3-W5, R\#7.D2).
\end{myquote}

\noindent
\textbf{Response.}
We have explained the absence of the comparison with relevant works in Section~\ref{sec:relatedWork}, where they cannot be directly compared with our system (R\#6.W2), reconstructed the paper by moving the workload generation algorithm (Algorithm 1) to Section~\ref{sec:indb_inference} (R\#6.W6), and further clarified the difference between our work and relevant works in Section~\ref{subsec:expSetup} (R\#7.D5).

Furthermore, we have added an "assumption" part in Section~\ref{sec:preliminaries} to discuss handling data schema   (R\#6.W5).
We also included additional experiments with new settings to evaluate our system. 
These include performance changes with new data updates (Figure~\ref{fig:insertion_workload_auc} and Figure~\ref{fig:insertion_workload_auc}) (R\#6.W3), performance on SPJ queries (Figure~\ref{fig:spj}) (R\#6.W3, R\#7.D2), and evaluation of the effectiveness of our system on a large Avazu dataset (Table~\ref{tab:mainstudy}) (R\#7.D2).

Please refer to our responses to R\#6.W2, R\#6.W6, R\#7.D5, R\#6.W3, R\#6.W4, R\#6.W5, R\#7.D2 below for the details.


%% Reviewer 1
\input{revision/R5}


%% Reviewer 2
\input{revision/R6}

%% Reviewer 3
\input{revision/R7}


\balance

\clearpage

\thispagestyle{empty}

\setcounter{page}{1}

\nobalance

==> tex/views/fig_sparsemax_flops.tex <==
\begin{figure}[t]
\centering
% \captionsetup{justification=centering}
\begin{subfigure}[b]{0.49\textwidth}
    \hspace{1mm}
    \centering
    \includegraphics[width=0.75\columnwidth]{figs/ExpertNumber/legend.pdf}
\end{subfigure}

\begin{subfigure}[b]{0.24\textwidth}
    \centering
    \includegraphics[width=0.97\columnwidth]{figs/ExpertNumber/sparsemax_ablation_payment_flops.pdf}
        \caption{Payment}
    \label{fig:sql}
\end{subfigure}
~
\begin{subfigure}[b]{0.24\textwidth}
    \centering
    \captionsetup{justification=centering,margin={0cm,0.7cm}}
    \includegraphics[width=0.97\columnwidth]{figs/ExpertNumber/sparsemax_ablation_credit_flops.pdf}
    \caption{Credit}
    \label{fig:db_scalability}
\end{subfigure}
\vspace{-5mm}
% \caption{Effects of $\alpha$-entmax and number of experts on efficiency.
% }
\caption{Effects of $\alpha$-entmax and \#experts on efficiency.}
\vspace{0mm}
\label{fig:exp_sparsemax_flops}
\end{figure}

==> todo.tex <==
 - Fig12b (Done)
 - IIS IDS bracket (Done)
 - NAS Reference. (Done)
 - IIS IDS mentioned in Section 4. (Done)
 - Reference. 
    - 53  (Done) 
    - 34  (Done)
    - 21  keep 
    - 59  (Done)
    - 60  (Done)

 - Fig 4 Caption (Done)
